AttriGuard: A Practical Defense Against Attribute Inference Attacks via Adversarial Machine Learning

Users in various web and mobile applications are vulnerable to attribute inference attacks, in which an attacker leverages a machine learning classifier to infer a target user's private attributes (e.g., location, sexual orientation, political view) from its public data (e.g., rating scores, page likes). Existing defenses leverage game theory or heuristics based on correlations between the public data and attributes. These defenses are not practical. Specifically, game-theoretic defenses require solving intractable optimization problems, while correlation-based defenses incur large utility loss of users' public data. In this paper, we present AttriGuard, a practical defense against attribute inference attacks. AttriGuard is computationally tractable and has small utility loss. Our AttriGuard works in two phases. Suppose we aim to protect a user's private attribute. In Phase I, for each value of the attribute, we find a minimum noise such that if we add the noise to the user's public data, then the attacker's classifier is very likely to infer the attribute value for the user. We find the minimum noise via adapting existing evasion attacks in adversarial machine learning. In Phase II, we sample one attribute value according to a certain probability distribution and add the corresponding noise found in Phase I to the user's public data. We formulate finding the probability distribution as solving a constrained convex optimization problem. We extensively evaluate AttriGuard and compare it with existing methods using a real-world dataset. Our results show that AttriGuard substantially outperforms existing methods. Our work is the first one that shows evasion attacks can be used as defensive techniques for privacy protection.

==> application.tex <==
\section{Evaluation  on Twitter}
\label{twitterexp}
%\myparatight{Human-in-the-loop Sybil detection}
%We apply SybilBlind to detect real Sybils in a  Twitter dataset.



 \myparatight{Twitter dataset} 
 We obtained a publicly available Twitter dataset with 1,000 Sybils and 10,000 benign nodes from Yang et al.~\cite{Yang12-spam}.
 This published dataset is a subset of the authors'  original one. 
 Since a Sybil can follow a large number of benign nodes without being followed back, 
 we transform this network to be an undirected one via keeping an edge between two nodes only if they 
 follow each other, which can reduce attack edges. 
 Then we extracted the largest connected component of the undirected network 
 since all compared methods work on connected networks. 
 
% We extracted the largest connected component of the undirected version of this dataset. 
%Specifically, each node is a Twitter user, and an edge between two nodes means that 
%the two nodes follow each other.
 
After preprocessing, we have 8,167 nodes in total, with 7,358 benign nodes and 809 Sybils. 
In other words, 9.9\% of nodes are Sybils. 
These Sybils are spammers that were  labeled by Yang et al.~\cite{Yang12-spam}.
In the Sybil region that consists of the 809 Sybils and edges between them, 
432 Sybils (53.4\%) are isolated from other Sybils, 
333 Sybils (41.2\%) form a large connected component,
and the remaining Sybils (5.4\%) form small connected components. 
The benign region and the Sybil region are densely connected. 
Specifically, each Sybil has 49 attack edges on average.



We note that it is challenging to obtain a dataset with labeled nodes.  
Although this Twitter dataset is relatively small,
its characteristics (e.g.,  the fraction of isolated Sybils, 
 the fraction of Sybils in the largest connected component in the Sybil region, 
and the large number of attack edges) are similar to those of 
a large-scale Twitter dataset studied by Ghosh et al.~\cite{Ghosh12}.
Therefore, we believe our results on this Twitter dataset are representative.

%For   social web services (e.g., Twitter~\cite{Ghosh12,Yang12-spam} and Renren~\cite{Yang11-sybil}), a large fraction of \emph{current} Sybils are isolated from other Sybils and the number of attack edges is relatively large comparing to the density in the benign region and the Sybil region. These measurement studies imply that, in these services,  propagation-based Sybil classification methods and SybilBlind cannot achieve satisfying classification performance at detecting current Sybils. In practice, online social networking service providers often hire human workers to manually inspect users and flag Sybils~\cite{sybilrank}. We will show that, even if the threat model required by SybilBlind is not  met, SybilBlind can still aid human workers to detect a large amount of Sybils via Sybil ranking. 


%We apply our SybilBlind and SybilNoise to iteratively aid human workers to detect Sybils in Twitter. As was shown by , a large fraction of current Sybils on Twitter are isolated from other Sybils and the number of attack edges is relatively large comparing to the density in the benign region and the Sybil region. These measurement studies imply that propagation-based Sybil classification methods cannot achieve satisfying classification performance at detecting current Sybils on Twitter. In practice, online social networking service providers often hire human workers to manually inspect users and flag Sybils~\cite{sybilrank}. We will show that, although the threat model required by SybilBlind is not completely met on Twitter, SybilBlind can still aid human workers to detect a large amount of Sybils via Sybil ranking. 



%In practice, online social networking service providers often hire human workers to manually inspect users and flag Sybils~\cite{sybilrank}. 
%SybilBlind  produces a ranking list of users for Sybil ranking, which can be used as a priority list for human workers. 

%In particular, we envision the 
%following iterative human-in-the-loop Sybil detection process in such online social networking services: in the very first iteration, there are no labeled nodes in the social network, and the service provider uses SybilBlind to produce a ranking list, of which the top-$K$ nodes  are  manually inspected by human workers to produce a set of labeled benign nodes and a set of labeled Sybils; in the $t$th iteration ($t>1$), the service provider uses SybilNoise to produce an updated ranking list of the remaining unlabeled nodes via taking all the nodes that are already manually labeled so far as an input to SybilNoise, and then human workers manually inspect the top-$K$ nodes of the updated ranking list.  The goal of such iterative Sybil detection is to maximize the number of Sybils that human workers can detect within the same number of iterations. 

%\myparatight{Twitter datasets} We will use two Twitter datasets with labeled real Sybils to evaluate the performance of the iterative human-in-the-loop Sybil detection. To better approximate trust relationships,  we keep an undirected edge between two users if and only if they follow each other. 
%
%Twitter-small. Describe the dataset, including size, edges, number of Sybils, the number of isolated Sybils, the density of the largest connected components. \\
%
%Twitter-large. Describe the dataset, including size, edges, number of Sybils, the number of isolated Sybils, the density of the largest connected components. \\



\myparatight{Refining our sampler using node features}
Previous studies~\cite{Yang11-sybil,Yang12-spam} found that Sybils  
proactively follow a large number of benign users in order to make more 
benign users follow them in various social networks,
 but only a small fraction of 
benign users will follow back.
Therefore, we extract the \emph{follow back rate} feature for each node in
the Twitter dataset (the original dataset is directed, so we can calculate the feature).
Then we rank all nodes according to their follow back rate features in an ascending order. 
Presumably, some Sybils (both isolated Sybils and Sybils from the largest connected Sybil component) 
will be ranked high and some benign nodes will be ranked low in the ranking list. 
Thus, we sample the subset $B$ from the bottom-$K$ nodes while we sample the subset 
$S$ from the top-$K$ nodes and we set $K=1000$ in our experiments. 
This sampler is more likely to sample nodes whose tentative labels have lower noises,
and thus it improves SybilBlind's performance. 
%Fig.~\ref{sybilranking} shows the fraction of Sybils in top 100-nodes intervals of the ranking list obtained using 
%the follow back rate feature. 

%, 74.6 of the top-1000 nodes are 
%Sybils and 100% of the bottom-1000 nodes are benign. 



\myparatight{Comparing with state-of-the-art approaches} 
We compare SybilBlind (without manual labels as a training dataset) with Sybil classification approaches SybilNoise and SybilBelief~\cite{sybilbelief} as well as Sybil ranking approaches SybilRank~\cite{sybilrank} and CIA~\cite{Yang12-spam}.
We assume 100 (around 1.2\% of all nodes)  nodes are sampled from the  network uniformly at random and are manually inspected to
get labels. These labels are used as a training dataset for SybilNoise, SybilBelief, SybilRank (can only leverage labeled benign nodes), and CIA (can only leverage labeled Sybils). 
We repeat the experiments over 10 times (in each time, a different set of 100 nodes are sampled and manually labeled). We found that SybilRank works worse than random ordering. 
Therefore, we set the restart probability of the random walk to be 0.15; 
we also use a restart probability of 0.15 for CIA, as recommended by its authors.
Table~\ref{twitterresults} shows the comparison results of Sybil classification, 
and Fig.~\ref{sybilranking} shows the comparison results of Sybil ranking, 
in which we divide top ranked nodes into 100-nodes intervals and measure the fraction of Sybils in each of them.

First, SybilBlind achieves low average FNRs and FPRs and is stable (i.e., standard deviations are small). 
The reason is that the benign nodes that are classified as Sybils together with the detected Sybils form a large connected component.  
 81\% of the benign nodes that are classified as Sybils link to at least one Sybil 
 and  70\% of Sybils that are classified as benign are isolated Sybils. 
% Table~\ref{falsepos} in Appendix shows details of the benign nodes that are classified to be Sybils by SybilBlind.

%we perform a \emph{t-test} to determine whether one method outperforms another. 
%Specifically, we say one method outperforms another if the \emph{p-value} is smaller than 0.05.
Second, SybilBlind achieves slightly better FPRs and substantially better FNRs than SybilNoise and SybilBelief.
%However, SybilBlind significantly outperforms SybilNoise and SybilBelief in terms of FNRs. 
The reason is that SybilBelief and SybilNoise highly rely on the representativeness of the manual labels, 
while SybilBlind repeats multiple 
sampling trials and automatically selects the sampling trial that achieves a good performance.  
In particular, we find that with certain sets of 100 sampled nodes,
 SybilBelief and SybilNoise can achieve performances that are comparable to SybilBlind.
However, for many sets of 100 sampled nodes, which are not representative samples of the benign nodes and Sybils, 
SybilBelief and SybilNoise achieve much worse performances. 
As a result, SybilBelief and SybilNoise have unsatisfying average performances and 
the performances are less stable. 

Third, SybilBlind also outperforms Sybil ranking methods. 
Again, we observe that SybilRank and CIA also rely on the representativeness of the manual labels, 
and their performances are unstable  
when  1.2\% of nodes are labeled. 
The fraction of Sybils in the 10th 
100-nodes interval is low for SybilBlind because 
we have 809 Sybils in total.


%We run SybilBlind without manual labels on this Twitter dataset over 10 times and report average results.
%In each run, we rank all nodes according to their aggregated probability of being a Sybil in a descending order. 
%Fig.~\ref{firstiteration} shows a sample ranking list and the average fraction of Sybils in top-$K$ nodes of the ranking lists. 
%We observe that SybilBlind is able to rank a large fraction of Sybils at the beginning of the ranking lists. 
%For instance, among the top-400 nodes, 91.5\% of them are Sybils.  
%%We find that XX\% of these Sybils are from the largest connected Sybil component. 
%
%
%Therefore, when applying SybilBlind, the service provider can flag top-$K$ nodes of the ranking list to be Sybils,
%which can detect reasonable number of Sybils while achieving a low FPR. 
%However, the key challenge is how to automatically determine the $K$ when
%the Sybil structure is unknown. 
% Figure~\ref{rankinglist} inspires us to leverage clustering techniques to determine $K$.
% Specifically, we use a clustering algorithm (e.g., k-means in our experiments) to group the nodes 
% according to their aggregated probability of being a Sybil; 
% we compute the average aggregated probability of being a Sybil for each cluster of nodes;
% and we predict that all nodes in the cluster with the largest average aggregated probability to be Sybils,
% i.e., $K$ is the number of nodes in this cluster.  
%Note that clustering methods often require the number of clusters to 
%be specified, and we automatically determine the number of clusters via the popular method called \emph{Gap Statistics}~\cite{gapstat}.
%Therefore, we design a method to automatically determine the number of clusters.
%Due to the limited space, we discuss our method in Appendix~\ref{cluster} and compare it with 
%conventional methods. 

\begin{table}[!t]\renewcommand{\arraystretch}{1}
\centering
\caption{Sybil classification on the Twitter dataset. Numbers in the parenthesis are standard deviations.}
\centering
%\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{|c|c|c|} \hline 
{\small Method} & {\small FPR} & {\small FNR}\\ \hline
{\small SybilBlind} & {\small 1.21\% (0.17\%)} & {\small 8.05\% (0.31\%)}\\ \hline
%{\small SybilBlind} & {\small 19.03\% (0.98\%)} & {\small 49.01\% (0.55\%)}\\ \hline
%{\small SybilBlind + labels} & {\small 1.11\% (0.06\%)} & {\small 7.96\% (2.15\%)}\\ \hline
%{\small SybilBlind + labels+ clustering} & {\small 1.31\% (0.05\%)} & {\small 4.04\% (1.95\%)}\\ \hline
{\small SybilNoise} & {\small 1.44\% (0.70\%)} & {\small 34.68\% (9.08\%)}\\ \hline
%{\small SybilNoise + clustering} & {\small 0.35\%(0.25\%)} & {\small 46.46\%(6.86\%)}\\ \hline
{\small SybilBelief} & {\small 1.45\% (0.71\%)} & {\small 34.80\% (9.10\%)}\\ \hline
%{\small SybilBelief + clustering} & {\small 0.37\%(0.25\%)} & {\small 46.97\%(6.89\%)}\\ \hline
%{\small SybilRank + clustering} & {\small 99.06\%(0.07\%)} & {\small 0.15\%(1.08\%)}\\ \hline
%{\small CIA + clustering} & {\small 50.45\%(49.16\%)} & {\small 35.07\%(31.42\%) }\\ \hline

\end{tabular}
%\vspace{-4mm}
\label{twitterresults}
\end{table}


\begin{figure}[t]
\center
%\vspace{-2mm}
%\subfloat[A sample ranking list]{\includegraphics[width=0.25 \textwidth]{Twitter-small-score-rank-curve.pdf}\label{rankinglist}}
{\includegraphics[width=0.455 \textwidth]{Top-100-nodes-interval.pdf}}
%\subfloat[Benign nodes in bottom-$K$ nodes]{\includegraphics[width=0.4 \textwidth]{Twitter-lcc-graph-by-group-bot-K-bi_100-bt_2-nb_5-ns_5-4combined.pdf}}
\vspace{-2mm}
\caption{Comparing with Sybil ranking methods.}
%Since we consider the scenario where no manual labels are available for training, 
%we sample 20 nodes uniformly at random,
%10 of which are treated as labeled benign nodes and 10 of which are treated as labeled Sybils. 
%SybilRank uses these ``labeled" benign nodes as a training dataset while SybilBelief uses the ``labeled" benign and Sybil nodes as a training dataset. }
\label{sybilranking}
%\vspace{-4mm}
\end{figure}


\begin{figure}[t]
\center
%\vspace{-2mm}
%\subfloat[A sample ranking list]{\includegraphics[width=0.25 \textwidth]{Twitter-small-score-rank-curve.pdf}\label{rankinglist}}
%{\includegraphics[width=0.4 \textwidth]{sybilrank-twitter.pdf}}
{\includegraphics[width=0.45 \textwidth]{SNoisevsSBlind_FNR.pdf}}
%\subfloat[Benign nodes in bottom-$K$ nodes]{\includegraphics[width=0.4 \textwidth]{Twitter-lcc-graph-by-group-bot-K-bi_100-bt_2-nb_5-ns_5-4combined.pdf}}
\caption{Performance of SybilNoise vs. the fraction of nodes that are manually labeled.}
%Since we consider the scenario where no manual labels are available for training, 
%we sample 20 nodes uniformly at random,
%10 of which are treated as labeled benign nodes and 10 of which are treated as labeled Sybils. 
%SybilRank uses these ``labeled" benign nodes as a training dataset while SybilBelief uses the ``labeled" benign and Sybil nodes as a training dataset. }
\label{stability}
%\vspace{-4mm}
\end{figure}


\myparatight{Number of manual labels SybilBelief/SybilNoise require to match SybilBlind's performance}
Fig.~\ref{stability} shows the FNRs of SybilNoise when a given fraction of nodes, which are sampled uniformly at random,
 are manually 
labeled to get a training dataset. Results of FPRs and SybilBelief  are similar, and thus we do not show them for simplicity.
We observe that SybilNoise and SybilBelief require manually labeling 25\%-30\% of nodes in order to achieve FNRs and FPRs that are comparable to SybilBlind. 
We determined whether two methods have a comparable performance using a \emph{t-test} 
with a significance level of 0.05. 
%Specifically, two methods have comparable performance if the \emph{p-value} is larger than 0.05 under t-test.
%Specifically, we perform a XX test to determine whether two methods achieve comparable (i.e., statistically 
%indistinguishable) performances. 
%The reason is that 


\myparatight{Summary} SybilBlind is accurate and stable on Twitter with real Sybils. State-of-the-art Sybil classification approaches require labeling a large training dataset to achieve comparable accuracy and stability with SybilBlind.  

%Table~\ref{twitterresults} shows the results on the Twitter dataset. 
%By combing SybilBlind with clustering, we can detect 46.91\% Sybils (i.e., FNR is 53.09\%) while achieving a FPR as low as 0.85\%.
%Moreover, XX\% and XX\% of the detected Sybils are from the largest connected Sybil component
%and isolated Sybils, respectively. 
%The reason we detect these isolated Sybils is that they, together with 
%the benign nodes that our method falsely labels as Sybils, are linked with the largest connected Sybil component to 
%form a bigger connected component. 

% Among the Sybils that
 
%\myparatight{Refining aggregator} We found that our HEA aggregator is sufficient when the social network has the homophily property. 
%However, the performance of HEA degrades when homophily is unsatisfied (see results in Table~\ref{}, which we will discuss soon). 
%To enhance SybilBlind, we refine the aggregator using clustering techniques. 
%Specifically, for each sampling trial in the top-$\kappa$ ones with the largest homophily,
%we rank the nodes according to their posterior probability of being a Sybil, from which we obtain
%a 



%\myparatight{Sybil classification} This Twitter follower-followee  network does not satisfy our threat model because a large fraction of Sybils are isolated from other Sybils and the number of attack edges is large.\footnote{We stress that this Twitter network uses follower-followee relationships. Other types of Twitter network (e.g., edges represent retweeting interactions) might satisfy the threat model.} Therefore, our SybilBlind (and other structure-based Sybil classification approaches requiring the homophily assumption) could achieve limited classification performance. Indeed, with default settings (refer to Section~\ref{exp-setup} for details) for the parameters, SybilBlind achieves a FNR 49\% and a FPR 8\%. This unsatisfying classification performance is not surprising since more than a half of Sybils are isolated from other Sybils in this Twitter dataset. 

%\myparatight{Sybil ranking} Although the Twitter network does not satisfy our threat model, 
%we show that SybilBlind can still achieve a very good Sybil ranking performance in terms of the Sybils in top-$K$ nodes (STK) and 
%benign nodes in bottom-$K$ nodes (BBK). 
%Again, we use default settings for the parameters of SybilBlind. 
%We compare SybilBlind with SybilRank and SybilBelief. 
%Since we consider the scenario where no manually labeled users are available as a training dataset, 
%we sample 20 users uniformly at random, and we treat 10 of them as labeled benign users and 
%the other 10 of them as labeled Sybils. The sampled users with noisy labels are used as a training dataset 
%for SybilRank and SybilBelief.
%We repeat the  experiments 10 times, 
%and we report the average results (we find the standard deviations are very small). 
% 
%
%Fig.~\ref{firstiteration} shows the fraction of Sybils in top-$K$ nodes and fraction of 
%benign nodes in bottom-$K$ nodes in the ranking lists
%produced by SybilBlind, SybilRank, and SybilBelief.
%First, we observe that SybilBlind substantially outperforms SybilRank and SybilBelief.
%Specifically, in the ranking list produced by SybilBlind, more than 90\% of the top-300 (i.e., around top 4\%) nodes are Sybils
% and 99.9\% of the bottom-4,000 (i.e., around bottom 50\%) nodes are benign. 
% This implies that, if the service provider only flags the top 4\% nodes as Sybils,
%  then the service provider can detect 34\% of Sybils 
%  while achieving a FPR that is as low as 0.4\%. 
%  %A low FPR is desired since falsely suspending 
%  %a benign user results in bad user experience and  
%
%Second, SybilRank is worse than random ordering in terms of both 
%Sybils in top-$K$ nodes and  benign nodes in bottom-$K$ nodes. 
%The reasons are  1) the Twitter dataset does not satisfy the homophily assumption  required by
%SybilRank, and 2) SybilRank is not robust to label noise.
%
%Third, SybilBelief's overall performance is close to random ordering.
%Specifically,  SybilBelief performs better than random ordering in terms 
%of Sybils in top-$K$ nodes while it performs worse than
%random ordering in terms of benign nodes in bottom-$K$ nodes. 
%The reason is that the average label noises in the benign region 
%and the Sybil region of the sampled nodes are 
%50\%.
%% which makes SybilBelief close to random ordering. 
%We note that we could extend our SybilBlind framework to SybilBelief to improve SybilBelief's performance. 
%Specifically, we can replace SybilNoise with SybilBelief in our framework, 
%and our homophily-entropy aggregator can identify the sampling trials in which SybilBelief achieves good performance.
%Since SybilBelief has similar robustness to label noises with SybilNoise, we expect 
%this extension will achieve similar Sybil ranking performance with SybilBlind.
%However, since SybilBelief is space and time inefficient, this extension will be unscalable. 

%\begin{figure}[t]
%\center
%%\vspace{-2mm}
%{\includegraphics[width=0.35 \textwidth]{Twitter-lcc-graphtop-K-sim-human-samplesize-comparison.pdf}}
%\caption{Fraction of Sybils in top-300 nodes as a function of the number of manually labeled nodes for SybilRank and SybilBelief.}
%%Since we consider the scenario where no manual labels are available for training, 
%%we sample 20 nodes uniformly at random,
%%10 of which are treated as labeled benign nodes and 10 of which are treated as labeled Sybils. 
%%SybilRank uses these ``labeled" benign nodes as a training dataset while SybilBelief uses the ``labeled" benign and Sybil nodes as a training dataset. }
%\label{compa}
%\vspace{-4mm}
%\end{figure}

%\myparatight{Number of manual labels  SybilRank and SybilBelief require to match SybilBlind's performance}
%Figure~\ref{compa} shows the performance of SybilRank and SybilBelief as a function of the number of manually labeled nodes. We assume the service provider samples nodes uniformly at random from the social network and asks human workers to label them. We observe that SybilBelief requires 90 (1.1\% of all nodes) manually labeled nodes in order to match SybilBlind's performance. SybilRank achieves bad performance even if we have manual labels. The reason might be that SybilRank cannot incorporate labeled Sybils. 



%\myparatight{Comparing with state-of-the-art approaches}
%We assume 100 nodes (around 1.1\% of all nodes) are  sampled from the network, 
%and they are manually inspected to get labels. So there are 90 labeled benign nodes
%and 10 labeled Sybils on average. 
%
%Table~\ref{twitterresults} shows the comparison results. The results are averaged over 10 runs.
%Note that SybilRank/CIA were designed to be Sybil ranking methods, and they require 
%human experts to manually inspect the produced ranking lists to detect Sybils.
%Therefore, we only show results for their combination with our clustering method.
% 
% We observe that our clustering method improves SybilBelief. 
% Moreover,
% SybilBlind + clustering significantly outperforms SybilBelief and SybilRank methods even if they use manual labels while 
% SybilBlind does not. 
%The reason is that SybilBelief/SybilRank relies on that the manual labels are representative samples of the benign nodes and Sybils, 
%while SybilBlind repeats multiple 
%sampling trials and automatically selects the sampling trial where a large fraction of Sybils are detected.  
%Specifically, Table~\ref{sybilbelief} shows three runs of SybilBelief + clustering, 
%in each of which 100 nodes are sampled from the Twitter network
%and are manually inspected to get labels. 
%We observe that SybilBelief's performance highly depends on the representativeness of manual labels,
%e.g., SybilBelief's performance is significantly different for different manual labels. 
%Therefore, its average performance over multiple runs is bad.
%This also implies that, in order to improve SybilBelief's performance and make it stable across manual labels,
%the service provider needs to  manually label even more nodes. 
 
  
%\begin{table}[!t]\renewcommand{\arraystretch}{1}
%\centering
%\caption{SybilBelief highly relies on representative manual labels.}
%\centering
%%\addtolength{\tabcolsep}{-4pt}
%\begin{tabular}{|c|c|c|} \hline 
%{\small Method} & {\small FPR} & {\small FNR}\\ \hline
%{\small SybilBelief + clustering, run 1} & {\small FPR} & {\small FNR}\\ \hline
%{\small SybilBelief + clustering, run 2} & {\small FPR} & {\small FNR}\\ \hline
%{\small SybilBelief + clustering, run 3} & {\small FPR} & {\small FNR}\\ \hline
%\end{tabular}
%%\vspace{-.1in}
%\label{sybilbelief}
%\end{table}


==> intro-cp.tex <==
\section{Introduction}
% MaLIA is important pervasive privacy threat. 

% Existing defenses and their limitations. 

% Our work: 1) privacy-risk metric, utility-loss metric, and problem formulation. 2) Our methods to solve the two problems. 3) Evaluations. 

\emph{Attribute inference attacks} are emerging threats to user privacy in various application domains ranging from social media~\cite{Zheleva09,Chaabane12,kosinski2013private,GongAttriInferSEC16} to recommender systems~\cite{Otterbacher10,weinsberg2012blurme} to mobile platforms~\cite{MichalevskyPowerSEC,Narain16Oakland}. 
In an attribute inference attack, an attacker aims to infer a user's {private attributes} (e.g., location, gender, sexual orientation, and/or political view) via leveraging its public data. 
In particular, the attacker has access to 1) a user's certain public data and 2) a machine learning classifier, 
which takes a user's public data as input and infers the user's private attributes.  
For instance, in social media, a user's public data could be the list of pages that the user liked on Facebook. Given these page likes, an attacker can use a machine learning classifier to accurately infer the user's various private attributes including, but not limited to, gender, sexual orientation, and political view~\cite{kosinski2013private}. 
 In recommender systems, a user's public data could be the list of items (e.g., movies, mobile apps, videos) that the user rated. Given the rating scores, an attacker can use a classifier to infer a user's gender with an alarming accuracy~\cite{weinsberg2012blurme}.  Attribute inference attacks can successfully infer a user's private attributes via its public data because users' private attributes are statistically correlated with their public data. 


%Some users do not view the attributes $A$ as private, so they also disclose them online. 
%The attacker can learn the machine learning classifier by using the data of users  

We represent a user's public data as a \emph{vector}. For instance, in recommender systems, an entry of the vector is the rating score the user gave to the corresponding item or 0 if the user did not rate the corresponding item. A defense against attribute inference attacks essentially adds noise to a user's public data vector (i.e., modify certain entries of the vector) with a goal to decrease the inference accuracy of an attacker. %, who has access to the noisy public data.
%Existing methods~\cite{weinsberg2012blurme,friendbasedDefense,ChenObfuscationPETS14} to defend against MaLIA essentially add noise to a target user's public data vector (i.e., modify certain entries of the vector) such that an attacker, who has access to the noisy public data, is less likely to accurately infer the user's private attributes.
%Due to the pervasive threats of MaLIA, various research communities are starting to develop defense methods against MaLIA~\cite{}. 
%A target user's public data are modeled as a \emph{vector}. 
%  These methods (including ours) essentially add noise to a target user's public data vector (i.e., modify certain entries of the vector) such that an attacker, who has access to the noisy public data, is less likely to accurately infer the user's private attributes.  However, different methods add the noises differently. 
One category of defenses (e.g.,~\cite{ShokriCCS12,Calmon:2012}) against inference attacks leverage game theory. In these methods, an attacker performs the optimal inference attack based on the knowledge of the defense, while the defender adds noise to the public data to defend against the optimal inference attack. These game-theory-based methods have theoretical privacy guarantees, but they are not practical for attribute inference attacks. Specifically, they formulate finding the noise as solving certain optimization problems, but the optimization problems are computationally intractable for the defender to solve, due to the high dimensionality of the public data in practice. 

Therefore, several studies~\cite{weinsberg2012blurme,friendbasedDefense,ChenObfuscationPETS14,Salamatian:2015} aimed to trade theoretical privacy guarantees for computational tractability. To be tractable, they either quantize the public data to reduce their dimensionality~\cite{Salamatian:2015} or  modify the entries that have large correlations with the private attribute values that do not belong to a user~\cite{weinsberg2012blurme,friendbasedDefense,ChenObfuscationPETS14}. However, these methods suffer from one or two key limitations. First, they~\cite{weinsberg2012blurme,friendbasedDefense,ChenObfuscationPETS14} require the defender to have direct access to a user's private attribute value, in order to compute the correlations between public data entries and private attribute values that do not belong to the user.  
Such requirement introduces usability issues and additional privacy concerns. Specifically, a user needs to specify its attribute value to the defender, which makes it inconvenient for users. Moreover, the defender becomes a single point of failure, i.e., when the defender is compromised, the private attribute values of all users are compromised. Second, as we will demonstrate in our experiments, they incur large utility loss, i.e., they add a large amount of noise to a user's public data. 

%Specifically, existing defense methods~\cite{weinsberg2012blurme,friendbasedDefense,ChenObfuscationPETS14} modify the entries that have large correlations with the private attribute values that do not belong to the  user. For instance,  Chen et al.~\cite{ChenObfuscationPETS14} %considered each entry of the public data vector is binary (e.g., they correspond to page likes, where 1 indicates the user liked the corresponding page and 0 indicates the user didn't), and they 
%proposed to modify the entries that are most likely to decrease the attacker's inference accuracy according to certain heuristics. 
%
%These methods suffer from three key limitations. First, they do not provide rigorous privacy guarantees.  %For instance, the authors of~\cite{ChenObfuscationPETS14} stated in their paper ``we do not aim to provide provable privacy properties". 
%One major reason is that they do not have a formal privacy-risk metric to measure the threat of MaLIA. Second, they require the defender to have direct access to a user's private attribute value, in order to compute the correlations between public data entries and private attribute values that do not belong to the user.  
%Such requirement introduces usability issue and additional privacy concerns. Specifically, a user needs to specify its attribute value to the defender, which makes it inconvenient for users. Moreover, the defender becomes a single point of failure, i.e., when the defender is compromised, the private attribute values of all users are compromised. Third, as we will demonstrate in our experiments, they achieve suboptimal privacy-utility tradeoffs, i.e., they need to add a large amount of noises to a user's public data to protect its private attributes. 
%
%We note that \emph{local differential privacy} (LDP)~\cite{RandomizedResponse,Kasiviswanathan:2008,DuchiLDP13,Erlingsson:2014,BassilySuccinctHistograms15,Fanti:2016,QinHeavyHitterCCS16,ShenPrivacyRecSysCCS16,smith2017interaction}, a notion based on differential privacy~\cite{Dwork:2006}, could also be applied to add noise to a  user's public data vector. 
%%LDP is used to obfuscate an individual user's data, i.e., public data in our case. 
%%LDP provides strong privacy guarantees. 
%However, LDP aims to achieve a privacy goal that is different from the one in MaLIA. 
%%Specifically, LDP's privacy goal is to add random noise to a target user's public data vector such that two arbitrary public data vectors have close probabilities (their difference is bounded by a privacy budget)   
%%to generate the same noisy public data vector. However, in defending against MaLIA, the privacy goal is to add noise to a target user's public data vector  
%%such that its private attributes cannot be accurately inferred by the attacker. 
%As a result, as we will demonstrate in our experiments, LDP achieves a suboptimal privacy-utility tradeoff at defending against MaLIA. We will discuss details of LDP in Section~\ref{relatedwork}.

\noindent
{\bf Our work:} We propose \emph{AttriGuard}, a practical defense against attribute inference attacks. AttriGuard is computationally tractable and incurs much smaller utility loss than existing  defense methods when reducing the attacker's inference accuracy by the same amount. 

%First, we formulate two \emph{inference-attack defense problems}. Second, we propose a two-phase framework MaLIAGuard to solve the two problems. Third, we extensively evaluate our framework and compare it with existing methods on a real-world dataset.

{\bf Problem formulation.} The defender adds random noise to users' public data, according to a \emph{noise-type-policy}, which specifies the types of noise that can be added. Different users may have different preferences on what types of noise can be added to their public data. For instance, in recommender systems, a user may prefer modifying its existing rating scores, or adding new rating scores to items the user did not rate before, or combination of them.  A {noise-type-policy} (e.g., Modify\_Exist, Add\_New, or Modify\_Add) is used to provide personalized defense services for users. The ultimate goal of the defender is to reduce an attacker's inference accuracy with a small utility loss of the public data. However, the defender faces two challenges at computing the attacker's inference accuracy: 1) no access to users' private attribute values (we consider this threat model to avoid single-point failure introduced by a compromised defender); and 2) no access to the attacker's classifier used to perform the attribute inference attack, since there are many possible choices for the classifier. 

To address the challenges, we consider an alternative goal for the defender. Specifically, the defender learns a classifier to perform attribute inference, e.g., using the data from the users who disclose both the public data and attributes. 
Since the defender adds random noise, the classifier's output is a random variable. The defender adds random noise such that the probability distribution of the classifier's output is close to a \emph{target probability distribution}, which is selected by the defender. For instance, the target probability distribution could be a uniform probability distribution over the possible attribute values, with which the defender aims to reduce the classifier's prediction to be close to random guessing. 



{\bf Problem formulation.} In our problem formulation, we have three parties: \emph{user}, \emph{defender}, and \emph{attacker}. A user wants to share a public data vector while maintaining secrecy of its certain attributes. 
Different users may have different preferences on what types of noises can be added to their public data. For instance, in recommender systems, a user may prefer modifying its existing rating scores, or adding new rating scores to items the user didn't rate before, or combination of them. Therefore, in our problem formulation, we define a \emph{noise-type-policy} (e.g., Modify\_Exist, Add\_New, or Modify\_Add), which specifies the types of noises that can be added and is used to provide personalized defense services for users.  
The defender adds random noise (also a vector) to a user's public data vector. The noise is generated according to a \emph{randomized noise addition mechanism} $\mathcal{M}$, which is a probabilistic mapping between public data vector and noise. For web services like social media or recommender systems, the defender can be a client-side browser extension, which acts on behalf of the user. 
 The attacker has access to the noisy public data. Since the noisy public data is randomized, the output of the attacker's classifier is also randomized. We denote the probability distribution of the randomized output over the possible attribute values as $\mathbf{q}=[q_1,q_2,\cdots]$, where $q_i$ is the probability that the classifier outputs the $i$th attribute value for the user. We note that, before accessing a user's noisy public data, an attacker could already have certain prior knowledge about the user's attributes. We model the prior knowledge as a \emph{prior probability distribution} $\mathbf{p}=[p_1,p_2,\cdots]$ over the possible attribute values. 
 
Essentially, defending against MaLIA is to find a $\mathcal{M}$ that achieves an optimal privacy-utility tradeoff. To this end, we need to define a privacy-risk metric and utility-loss metric. 
Intuitively, a user's privacy risk is small if observing the noisy public data only slightly increases an attacker's information about the user's private attribute value, compared to the prior probability distribution that the attacker already has. Therefore, we use information gain of the attacker's classifier's output (i.e., the information about the user's private attribute value, which an attacker has after observing the noisy public data) over the prior probability distribution as the privacy risk.
%It is challenging to define a privacy-risk metric to measure the threat of MaLIA to a user because 1) the defender does not have access to the user's true attribute value and 2) adding noise to the user's public data cannot change the attacker's prior probability distribution. To address these challenges, we use  information gain of the classifier's output over the prior probability distribution as the privacy risk. Intuitively, a user's privacy risk is small if observing the noisy public data only slightly increases an attacker's information about the user's private attribute value. 
Formally, we capture the information gain (and thus the privacy risk) by the Kullback--Leibler (KL) divergence between  $\mathbf{p}$ and $\mathbf{q}$. In principle, we can use any distance metric between the true public data vector and the noisy public data vector to measure utility loss. However, in this work, we focus on using the $L_0$ norm of the noise vector as an utility-loss metric because this metric characterizes the number of entries of the public data vector that are modified by the defender, which has intuitive and semantic interpretations in many application domains.  Given the privacy-risk metric and utility-loss metric, we formulate two versions of \emph{Inference-Attack Defense Problem}. Specifically, in the Inference-Attack Defense Problem I (or II), given a noise-type-policy and a privacy-risk budget (or an utility-loss budget), we aim to find a randomized noise addition mechanism, with which the user's privacy risk (or utility loss) is less than the budget while utility loss (or privacy risk) is minimized. %In the Inference-Attack Defense Problem II, given a noise-type-policy and an utility-loss budget, we aim to find a randomized noise addition mechanism, with which the user's utility loss is less than the budget while privacy risk is minimized.


{\bf  Two-phase framework MaLIAGuard.} We propose a two-phase framework to solve the two versions of Inference-Attack Defense Problem. Specifically, we consider four scenarios depending on whether the defender knows the attacker's prior probability distribution $\mathbf{p}$ and classifier: Scenario I (known $\mathbf{p}$ and known classifier), Scenario II (unknown $\mathbf{p}$ and known classifier), Scenario III (known $\mathbf{p}$ and unknown classifier), and Scenario IV (unknown $\mathbf{p}$ and unknown classifier). %Our two-phase framework is applicable to all the four scenarios. Specifically, 
 For Scenario I, in Phase I, we leverage \emph{adversarial machine learning} to find noises to evade the attacker's classifier. In particular, for each possible attribute value $i$, we find the minimal noise $\mathbf{r}_i$ such that the classifier predicts $i$ for the user's attribute when taking the noisy public data as input. This is known as \emph{evasion attacks} to machine learning~\cite{barreno2006can,laskov2014practical,Goodfellow:ICLR:14b,Papernot:arxiv:16Limitation,XuEvasionMalware,sharif2016accessorize}. However, existing evasion attack methods are insufficient to find the noises in our problem, because they do not consider different noise-type-policies. Therefore, we propose a new evasion attack method to find the noises. Our method is based on the saliency map technique developed by Papernot et al.~\cite{Papernot:arxiv:16Limitation}. Evasion attacks are often viewed as offensive techniques. Our work demonstrates that evasion attacks can also be used as defensive techniques. In particular, evasion attacks can play an important role at defending against MaLIA. In Phase II, we model the randomized noise addition mechanism $\mathcal{M}$ as a probability distribution over the noises $\mathbf{r}_1$, $\mathbf{r}_2$, $\cdots$. Then, we obtain $\mathcal{M}$ via solving convex optimization problems. For Scenario II, we estimate the upper bound of privacy risk for any prior probability distribution. We then use the upper bound to compute $\mathcal{M}$ using our two-phase framework, which means that we want to achieve a privacy-utility tradeoff for any prior probability distribution. Moreover, we transform Scenario III (or IV) to Scenario I (or II) via learning a classifier using data publicly available to approximate the attacker's classifier. %In Phase I, the defender computes the noises with respect to the learnt classifier. Such noises are highly likely to be applicable to the attacker's classifier, which is known as \emph{transferability} in adversarial machine learning~\cite{}. The classifier learnt by  


{\bf Evaluations.} We evaluate our framework and compare it with existing methods using a real-world dataset from the reputation system domain. A user's public data are the rating scores the user gave to mobile apps on Google Play; and the attribute is the city a user lives/lived in. First, our results demonstrate that our evasion attacks outperform existing ones in Phase I of our framework. Second, our framework achieves good privacy-utility tradeoffs. For instance, by modifying at most 2 rating scores on average, the attacker's inference accuracy is reduced by 75\%; and the inference accuracy of the classifier is close to that of using the prior probability distribution, which means that  the noisy public data are rendered useless at increasing the attacker's knowledge about users' private attributes. 
Third, our framework achieves similar privacy-utility tradeoffs for the four scenarios, which means that whether the defender knows the attacker's prior knowledge and classifier does not significantly impact the defense effectiveness. Fourth, our framework achieves substantially better privacy-utility tradeoffs than existing methods. 
%For instance, 


%With increasing volumes of user data are being collected by third party who aim to provide personalized services or targeted advertising to users, such as intelligent personal assistant(like Siri) and recommendation systems. 
%However, the collection of user's data could incur significant privacy risk. There has been a fair amount of work indicating that user demographics information such as age, gender, ethnicity or even sexual orientation could be inferred using statistical inference attack by third party. 
%For example, the location of user could be infer by sensor data of the mobile ~\cite{Narain:SP:16}.
%Consequently, the concerns about privacy has spurred the research in the field of theoretical models as well as the application to the design of the privacy preserving system. 
%Without such system, user in the future might stop using those services and thus, it would be hard for companies to improve personal experience of the product due to privacy law constraints as well user concerns. 
%
%One fundamental problem in design a privacy preserving system is how to make the right tradeoff between privacy and utility. 
%A majority of techniques has been proposed to resolve the tensions between utility and privacy loss, such as anonymization, k-anonymity and differential privacy.  Those perturbation techniques 
%are based on some form perturbation of the data which result in utility privacy tradeoff. However, those approaches cannot directly applied in practce due to various reason such as adding too much noise, the need of trustful third party which is impractical., computation inefficient and so on.
%
%To address the deficiency of the existing solutions, we propose APSI, a general privacy preserving framework based on information-theoretic as well as the adversarial machine learning against statistical inference attack. 
%We consider both situations of \emph{Know Prior Attack} as well as \emph{Unknow Prior Attack}. We analysize the utility loss given privacy budget or privacy loss given utility budget in those situations. 
%More importantly, we don't need to assume there are trustful third party, i.e., we don't need to user provide their private information. 

In summary, our key contributions are as follows:
\begin{itemize}
\item We formulate the problem of defending against machine learning based inference attacks. 

\item We propose a framework to solve the inference-attack defense problems in different scenarios. 

\item We extensively evaluate our framework and compare it with existing methods using a real-world dataset.

\end{itemize}




==> model.tex <==
\section{Design of AttriInfer}
\subsection{Overview}
Suppose we consider a binary attribute $A$. 
Given a training dataset, we first use user behaviors to learn a binary classifier for the attribute. 
Then, we use the classifier to predict the probability that each target user has the attribute $A$. 
We call this probability \emph{prior probability}. 
We use a binary random variable to model each user, and we model the joint probability distribution of all binary random variables as a pairwise Markov Random Field (pMRF) based on the structure of the social network. 
Given the training dataset and prior probability, we propagate label information among the social graph via the pMRF model. After the propagation, we obtain a posterior probability of having the attribute for each target user. Then, we use the posterior probability to predict whether a target user has the attribute or not. In this section, we introduce a basic version of AttriInfer, in which we use Loopy Belief Propagation (LBP) to infer the posterior probabilities. 



\subsection{Learning Prior using Behaviors}
We associate a binary random variable $x_u$ with each user $u$, where $x_u=1$ means that $u$ has the attribute $A$ and $x_u=-1$ means that $u$ does not have the attribute. %$\bar{x}_u$ indicates the observed value 
We denote the behaviors of a user $u$ as a \emph{behavior vector} $\vec{b}_u$. The vector $\vec{b}_u$ can be a binary vector, where an entry is 1 if and only if $u$ has performed a certain action on the corresponding object. For instance, when we consider page likes as behaviors, an entry of 1 means that the user liked the corresponding page. The behavior vector $\vec{b}_u$ can also be a real-valued vector. For instance, when we consider reviews as behaviors, an entry is the rating score that a user gave to the corresponding item (e.g., app, movie, book). Likewise, when we consider {clickstream} as behaviors, an entry of a user's behavior vector can be the frequency of a certain subsequence (consisting of click events and discretized time gaps between them) that appears in the user's clickstream~\cite{Wang13Clickstream,WangCHI16}. 


We learn the prior probability of target users using a standard {logistic regression classifier}.
Specifically,  the probability $q_u$ that  $u$ has the attribute $A$ is modeled as $q_u=Pr(x_u=1)=\frac{1}{1 + exp(-h_u)}$, where $h_u=\vec{b}_u ^T\cdot \vec{c} + d$.  $d$ and the vector $\vec{c}$ are parameters of the logistic regression classifier. 
Given a training dataset, in which each user has behaviors,  we can learn these parameters via \emph{maximum likelihood estimation}. In our experiments, we leverage the library LIBLINEAR~\cite{liblinear08} to learn these parameters.  We note that we choose logistic regression classifier instead of a Support Vector Machine (SVM) because SVM does not directly produce a probability that a user has the attribute.\footnote{We note that SVM's outputs can be transformed into probabilities~\cite{liblinear08}, but they achieve suboptimal performance.} With this logistic regression classifier, we can compute the prior probability for each user who has behaviors. 
A user has a prior probability of 0.5 if it does not have behaviors.
%  has a prior probability of 0.5. %For a training user who has the attribute, we set its prior probability to be close to 1 (e.g., 0.9 in our experiments)
%For a users in the training dataset, we set 

\subsection{Propagating Prior Using Social Graph}
 We leverage a pMRF to model the social graph, with which we can propagate the prior probability among the social graph to compute a posterior probability that each target user has the attribute. 
\subsubsection{Intuitions} 
We  denote by $\Gamma_u$ the set of  $u$'s neighbors in the social network, and $\bar{x}_{\Gamma_u}$ the observed states (whether having the attribute or not) of the neighbors. 
Social networks are known to have the \emph{homophily} property~\cite{homopily01}, i.e., if we sample an edge $(u,v)$ from a social graph uniformly at random, the two users $u$ and $v$ are highly likely to both have the attribute or both not have the attribute. Based on this homophily intuition, we model the probability that a user $u$ has the attribute $A$ 
when the user's neighbors' states are already known  
as follows:
\begin{align}
\label{local_rule}
Pr(x_u=1|\bar{x}_{\Gamma_u})=\frac{1}{1+\text{exp}(-\sum_{v\in \Gamma_u}J_{uv}\bar{x}_v - h_u)} \ ,
\end{align}
where $J_{uv} > 0$ is the homophily strength between $u$ and $v$, and $h_u$ characterizes $u$'s  prior knowledge obtained through the logistic regression classifier.  A higher $J_{uv} $ means that $u$ and $v$ are more likely to have the same state. 


%Specifically, $J_{uv}>0$ means $u$ and $v$ tend to have the same state;  $J_{uv}<0$ indicates $u$ and $v$ tend to have opposite states; and $J_{uv}=0$ indicates that there is no coupling between them. In practice, these coupling strengths can encode trust levels between nodes. 
%%In these variables we encode our general homophily assumption, i.e. we set them to a global (independent from $u$,$v$) positive value.
%
%Note that our local rule in Equation~\ref{local_rule} incorporates the homophily assumption via setting $J_{uv}>0$.
%
 

\subsubsection{A Pairwise Markov Random Field}
We find that Equation~\ref{local_rule} can be achieved by modeling the social graph as a pairwise Markov Random Field (pMRF). A pMRF defines a joint probability distribution for binary random variables associated with all the users in the social graph. Generally speaking, a pMRF is specified by a \emph{node potential} for each user $u$, which incorporates prior probability about $u$, and an \emph{edge potential} for each edge $(u,v)$, which represents correlations between $x_u$ and $x_v$.  In our attribute inference problem, we define a node potential $\phi_u(x_u)$ for user $u$ as
\begin{displaymath}
\phi_u(x_u):=
\begin{cases} 
q_u  & \text{if } x_u = 1  \\ 
1-q_u  &  \text{if } x_u = -1
\end{cases} 
\end{displaymath}
and an \emph{edge potential  $\varphi_{uv}(x_u, x_v)$} for the edge $(u,v)$ as
\begin{displaymath}
\varphi_{uv}(x_u, x_v):=
\begin{cases} 
w_{uv} & \text{if } x_u x_v = 1  \\  
1 - w_{uv} &  \text{if } x_u x_v = -1 \ ,
\end{cases}
\end{displaymath}
where $w_{uv}\!:=\!(\!1+\!\mathrm{exp}\{-J_{uv}\})^{-1}$. 
Then, the following pMRF satisfies Equation~\ref{local_rule} for every user.
$$Pr(x_V)= \frac{1}{Z}\prod_{u\in V} \phi_u(x_u) \prod_{(u, v)\in E} \varphi_{uv}(x_u, x_v)\ ,$$
where $Z=\sum_{x_u}\prod_{u\in V} \phi_u(x_u) \prod_{(u, v)\in E} \varphi_{uv}(x_u, x_v)$ is called the partition function and normalizes the probabilities.
%The  edge potential $\varphi_{uv}(x_u, x_v)$ encodes the homophily strength of two linked users $u$ and $v$. The larger $w_{uv}$ is, the stronger the model favors $u$ and $v$ to have the same state.   More precisely,  $w_{uv} > 0.5$ means connected nodes tend to have the same state; $w_{uv} < 0.5$ means connected nodes tend to have opposite states; $w_{uv}=0.5$ encodes the scenario where there is no coupling between $u$ and $v$.  Note that setting $w_{uv} > 0.5$ encodes our homophily assumption.
$w_{uv} > 0.5$ captures the homophily property.  
In our definitions, $w_{uv}$ can be interpreted as the probability that two linked users  have the same state. In this work, we set $w_{uv}=w>0.5$ for all edges, and we call $w$ \emph{homophily strength}.  
However, learning the parameters $w_{uv}$ for different edges would be a valuable future work. 

\subsubsection{Estimating Posterior Probability using LBP}
We compute the \emph{posterior probability distribution} of a user $u$, i.e., 
$Pr(x_u) = \sum_{x_{V/u}} Pr(x_V)$. For simplicity, we denote by $p_u$ the posterior probability that 
$u$ has the attribute, i.e., $p_u=Pr(x_u=1)$.  
 This posterior probability is used to predict whether a user has the attribute or not.  
In the basic version of AttriInfer, we use Loopy Belief Propagation (LBP)~\cite{Pearl88} to estimate the posterior probability distribution $Pr(x_u)$. 
LBP iteratively passes messages between neighboring users in the graph. Specifically, the message $m_{vu}^{(t)}(x_u)$ sent from $v$ to $u$ in the $t$th iteration is 
\begin{align}
\label{message}
m_{vu}^{(t)}(x_u) = \sum_{x_v} \phi_v (x_v) \varphi_{vu}(x_v, x_u) \prod_{k \in \Gamma(v)/u} m_{kv}^{(t-1)}(x_v),
\end{align} 
where $\Gamma(v)/u$ is the set of all neighbors of $v$, except the receiver node $u$. This encodes that each node %essentially
 forwards a product over  incoming messages of the last iteration and adapts this message to the respective receiver based on the homophily strength with the receiver. LBP stops when the changes of messages  become negligible in two consecutive iterations (e.g., $l_1$ distance of changes becomes smaller than $10^{-3}$) or it reaches the predefined maximum number of iterations $T$. After LBP halts, we estimate the posterior probability distribution $Pr(x_u)$ as follows:
 \begin{align}
 \small
 \label{posteriorfull}
 Pr^{(t)}(x_u)\propto \phi_u (x_u) \prod_{k \in \Gamma(u)} m_{ku}^{(t)}(x_u),
 \end{align} 
which is equivalent to
\begin{align}
 \label{belief}
 \begin{split}
 & p_u^{(t)}=\frac{q_u \prod\limits_{k \in \Gamma(u)} m_{ku}^{(t)}}{q_u \prod\limits_{k \in \Gamma(u)} m_{ku}^{(t)} + (1-q_u) \prod\limits_{k \in \Gamma(u)} (1-m_{ku}^{(t)})}, \\
 \end{split}
 \end{align} 
 where $m_{ku}^{(t)}=m_{ku}^{(t)}(x_u=1)$ and $1-m_{ku}^{(t)}=m_{ku}^{(t)}(x_u=-1)$.
 Note that normalizing $m_{ku}^{(t)}(x_u)$ does not affect the computation of posterior probability distribution of any user. 
 Therefore, for simplicity, we have normalized  $m_{ku}^{(t)}(x_u)$ such that  $m_{ku}^{(t)}(x_u=1)$ + $m_{ku}^{(t)}(x_u=-1)=1$ in the above equation. 

We note that pMRF and LBP were also adopted to detect Sybils in OSNs~\cite{sybilbelief}. 
Sybil detection and attribute inference for binary attributes are algorithmically similar. 
However, previous work~\cite{sybilbelief} didn't perform optimization and convergence analysis as we will discuss 
in the next two sections Section~\ref{optimization} and Section~\ref{sec:cvgAnal}.  

\section{Optimizing AttriInfer}
\label{optimization}
The basic version of AttriInfer has two shortcomings: 
1) AttriInfer is not scalable enough, and 2) AttriInfer is an iterative method but is not guaranteed to converge. 
Being not convergent makes it hard to select an appropriate number of iterations. 
The reason is that LBP maintains messages on each edge and  LBP might oscillate on loopy graphs~\cite{Pearl88}.
Therefore, we further optimize AttriInfer to address these shortcomings. 

\subsection{Eliminating Message Maintenance}
One of the major reasons why basic AttriInfer is not scalable enough is that LBP maintains messages on each edge. 
We observe that the key reason why LBP needs to maintain messages on edges is that  when  a node $v$ prepares a message to its neighbor $u$, it excludes the message that $u$ sent to $v$.  
Therefore, our first optimization step is to include the message that $u$ sent to $v$ when $v$ prepares its message for $u$. 
Formally, we approximate Equation~\ref{message} as:
\begin{align}
%\label{message}
m_{vu}^{(t)}(x_u) = \sum_{x_v} \phi_v (x_v) \varphi_{vu}(x_v, x_u) \prod_{k \in \Gamma(v)} m_{kv}^{(t-1)}(x_v).
\end{align} 

Considering Equation~\ref{posteriorfull}, we have:
\begin{align}
m_{vu}^{(t)}(x_u) \propto \sum_{x_v} \varphi_{vu}(x_v, x_u) Pr^{(t-1)}(x_v).
\end{align}
Recall that we normalize  $m_{vu}^{(t)}(x_u)$ such that  $m_{vu}^{(t)}(x_u=1)$ + $m_{vu}^{(t)}(x_u=-1)=1$, and we abbreviate $m_{vu}^{(t)}(x_u=1)$ as $m_{vu}^{(t)}$.  With such normalization,  our new messages become:
\begin{equation}
\small
\label{modifiedMessage}
m_{vu}^{(t)} = p_v^{(t-1)} w + (1-p_v^{(t-1)})(1-w).
\end{equation}
AttriInfer does not need to maintain messages on edges using our new messages. 

\subsection{Linearizing as a Matrix Form} 
AttriInfer iteratively applies Equations~\ref{modifiedMessage} and~\ref{belief} using our new messages,
which still cannot guarantee convergence. 
The key reason is that Equation~\ref{belief} combines messages from a user's neighbors \emph{nonlinearly}. 
We make AttriInfer converge via linearizing Equation~\ref{belief}. 
The resulting optimized AttriInfer can be represented in a concise matrix form. 
Before introducing our linearization, we define some terms. 
In particular, we define the \emph{residual} $\hat{y}$ of a variable $y$ as $\hat{y}=y-0.5$; 
and we define the \emph{residual vector} $\hat{\mathbf{y}}$ of $\mathbf{y}$ as $\hat{\mathbf{y}} = [y_1-0.5, y_2-0.5, \cdots]$.


%\begin{definition}[Residual Variable and Vector] 
%\label{def_1}
%We define the residual of a variable $y$ as $\hat{y}=y-0.5$; 
%and we define the residual vector $\hat{\mathbf{y}}$ of $\mathbf{y}$ as $\hat{\mathbf{y}} = [y_1-0.5, y_2-0.5, \cdots]$.
%and we define the residual matrix $\hat{\mathbf{Y}}$ of $\mathbf{Y}$  as each entry of $\mathbf{Y}$ substracting 0.5.
%\end{definition}




%\begin{lemma}[Residual Messages] The residual message $\hat{m}_{vu}^{(t)}$ can be represented as follows:
%\label{lemma_1}
%%With above denotation, we have
%\begin{equation}
%\small
%\label{res_nei_influ_sybil}
%\hat{m}_{vu}^{(t)} = 
%\begin{cases} 
%0 & \text{if } \hat{p}_v^{(t-1)}  > 0 \text{ and } v \in \Gamma_{i} (u) \\
%0 & \text{if } \hat{p}_v^{(t-1)}  < 0 \text{ and } v \in \Gamma_{o} (u) \\
%2 \hat{p}_{v}^{(t-1)} \hat{w} &\text{otherwise}.
%\end{cases} 
%\end{equation}
%\end{lemma}
%
%\begin{proof}
%By substituting variables in Eqn.~\ref{modifiedMessage} with their residuals.
%\end{proof}

%We denote by $\mathbf{A}_b\in \mathbb{R}^{|V| \times |V|}$, $\mathbf{A}_i\in \mathbb{R}^{|V| \times |V|}$, and $\mathbf{A}_o\in \mathbb{R}^{|V| \times |V|}$ the bidirectional, unidirectional incoming, and unidirectional outgoing adjacency matrices of the social graph, respectively. 
%The $u$th row of $\mathbf{A}_b$, $\mathbf{A}_i$, and $\mathbf{A}_o$ represents the bidirectional, unidirectional incoming, and unidirectional outgoing neighbors of $u$. Formally, if there exists a bidirectional edge between $u$ and $v$, then the entry $A_{b,uv}=A_{b,vu}=1$, otherwise, $A_{b,uv}=A_{b,vu}=0$;
%if there exists an unidirectional edge from $u$ to $v$, then $A_{o,uv}=1$ and $A_{i,vu}=1$.
 
For convenience, we denote by $\mathbf{p}^{(t)} = [p_1^{(t)} ; p_2^{(t)} ; \cdots; p_{|V|}^{(t)} ]$ a column vector all users' posterior probability in the $t$th iteration, and its residual vector as $\hat{\mathbf{p}}^{(t)} $. Similarly, we denote by a column vector $\mathbf{q}  = [q_1; q_2; \cdots; q_{|V|}]$ all users' prior probability,  and by $\hat{\mathbf{q}} $ its residual vector. Moreover, we denote by $\mathbf{M}\in \mathbb{R}^{|V| \times |V|}$ the adjacency matrix of the social graph. 
 %Let $\hat{\mathbf{P}}^{(t)} \in \mathbb{R}^{|V| \times |V|}$ be a matrix consisting of $|V|$ repeats of the column vector $\hat{\mathbf{p}}^{(t)} $, i.e., $\hat{\mathbf{P}}^{(t)}  = [\hat{\mathbf{p}}^{(t)} , \hat{\mathbf{p}}^{(t)} , \cdots]$. 
With these notations, we can approximate AttriInfer as a concise matrix form. Formally, we have the following theorem. 

%We define $\mathbf{p} = [p_1; p_2; \cdots; p_{|V|}]$ as the column vector of all nodes' posterior beliefs, and $\hat{\mathbf{p}}$ as its residual vector. Similarly, we denote by $\mathbf{q} = [q_1; q_2; \cdots; q_{|V|}]$ the column vector of all nodes' prior beliefs.  and by $\hat{\mathbf{q}}$ its residual vector. 
%
%With these notations and By setting all $w_{vu}$ as a fixed $w$, we have the following theorem regarding the approximate GANG.


% We further define $\mathbf{Q}=[\mathbf{q}_{1}; \mathbf{q}_{2}; \cdots ; \mathbf{q}_{|V|} ] = [\mathbf{q}(1), \mathbf{q}(-1)] \in \mathbb{R}^{|V| \times 2}$ and $\mathbf{P}=[\mathbf{p}_{1}; \mathbf{p}_{2}; \cdots ;  \mathbf{p}_{V}] = [\mathbf{p}(1), \mathbf{p}(-1)] \in \mathbb{R}^{|V| \times 2}$; their residual matrices are $\hat{\mathbf{Q}}=[\hat{\mathbf{q}}(1), \hat{\mathbf{q}}(-1)]$ and $\hat{\mathbf{P}}=[\hat{\mathbf{p}}(1),\hat{\mathbf{p}}(-1)]$. With such definitions, we have the following theorem regarding the approximate GANG.

\begin{theorem}
\label{theorem_1}
%Denote $\mathbf{A} \circ \mathbf{B}$ as the Hadamard (element-wise) product of matrix $\mathbf{A}$ and $\mathbf{B}$. 
%Furthermore, we set $\hat{\mathbf{p}}^{(0)} = \hat{\mathbf{q}}$. 
We can approximate Equations.~\ref{modifiedMessage} and~\ref{belief}  as the following equation: 
%the final residual belief vector $\hat{\mathbf{p}}$ can be approximated by iteratively solving the following equations
\begin{equation}
\label{approx_update}
\hat{\mathbf{p}}^{(t)} = \hat{\mathbf{q}} + 2\cdot\hat{w}\cdot \mathbf{M} \cdot \hat{\mathbf{p}}^{(t-1)}.
\end{equation}
%where the operator $\circ$ represents element-wise product of two matrices, $\mathbf{Y}^T$ is the transpose of the matrix $\mathbf{Y}$, and the indicator function $I(\mathbf{Y})$ means that an entry is set to be 0 if the corresponding entry of the matrix $\mathbf{Y}$ is non-negative, otherwise it is set to be 1. 
%  means setting positive entries of matrix $\mathbf{Y}$ to be 0, and $\mathbf{Y}(\mathbf{Y}<0)=0$ means setting negative entries of matrix $\mathbf{Y}$ to be 0. 
\end{theorem}
\begin{proof}
See Appendix~\ref{app:theorem1}.
\end{proof}

Theorem~\ref{theorem_1} enables us to design an efficient version of AttriInfer: first, we learn the prior probability for each user using behaviors; second, we iteratively apply Equation~\ref{approx_update} to compute the posterior probabilities for all target users simultaneously. AttriInfer halts when the relative change of the posterior probability vector in two consecutive iterations is smaller than $10^{-3}$.

We note that Gatterbauer et al.~\cite{gatterbauer2015linearized} also linearized LBP over a pMRF, and their linearized version is similar to ours. However, their linearization requires different heuristics and assumptions. For instance, their linearization requires residual of the homophily strength to be very small and the approximation of $\frac{\frac{1}{k}+\epsilon_1}{1+\epsilon_2}\approx \frac{1}{k} +\epsilon_1 -\frac{\epsilon_2}{k}$ when $\epsilon_1$ and $\epsilon_2$ are very small. In contrast, our linearization does not require these assumptions/approximations. Moreover, we eliminate message maintenance before linearizing Equation~\ref{belief}, which makes linearization much simpler, while their approach does not.

 
%demonstrates that posterior beliefs can be iteratively solved by matrix operations without explicitly modeling messages. 
%\textbf{Algorithm 2} summarizes our optimized version of GANG (GANG\_Opt). We note that Gatterbauer et al.~\cite{gatterbauer2015linearized} linearized LBP for a standard pMRF modeling an undirected graph, 
%while our work linearizes LBP for a new pMRF modeling a directed graph. 

%Note that above update equations directly calculate beliefs, i.e., without storing the passing messages. Moreover, the update can converge after several iterations (See Section VI). In doing so, we then predict $u$ to be a fraudulent node if $\hat{p}_u(1) > 0 $. For simplicity, we denote such approximate GANG as GANG\_Appr and illustrate its algorithmic procedure in \textbf{Algorithm 2}. 

%\begin{algorithm}[!htb]
%\caption{Optimized version of GANG (GANG\_Opt)}
%\label{alg:GANG}
%\begin{algorithmic}
%\REQUIRE $G=(V,E)$, $L_f$, $L_n$, $\epsilon$, $w$, $\delta=10^{-3}$, and $T=20$. \\
%\ENSURE  $p_u, \forall \, u \in V$. \\
%    Initialize $\hat{\mathbf{p}}^{(0)} = \hat{\mathbf{q}}$. \\
%    Initialize $t=1$. \\
%%\noindent \textbf{Process:}
%%\PROCESS ~~\\
%    %\WHILE { $\sum_{u\in V}|\hat{{p}}_u^{(t)} - \hat{{p}}_u^{(t-1)}| \geq \delta$ and $t \leq T$} \;
%    \WHILE { $\frac{\|\hat{\mathbf{p}}^{(t)} - \hat{\mathbf{p}}^{(t-1)}\|_1} {\|\hat{\mathbf{p}}^{(t)}\|_1} \geq \delta$ and $t \leq T$} \;
%    \STATE Update residual belief vector $\hat{\mathbf{p}}^{(t)}$ using Eqn.~\ref{approx_update}; \\
%    \STATE  $t=t+1$. \\
%    \ENDWHILE \\
%    \RETURN $\hat{\mathbf{p}}^{(t)} + 0.5$. \\
%\end{algorithmic}
%\end{algorithm}

 
 
 \section{Theoretical Analysis}
 \subsection{Convergence Analysis}
\label{sec:cvgAnal}
We analyze the condition when the optimized version of AttriInfer converges. Such analysis guides us to select appropriate homophily strength $w$.
Suppose we are given an iterative linear process: $\mathbf{y}^{(t)} \leftarrow \mathbf{c} + \mathbf{D} \mathbf{y}^{(t-1)}$. 
According to~\cite{saad2003iterative}, the linear process converges with any initial choice $\mathbf{y}^{(0)}$ if and only if the \emph{spectral radius} of the matrix $\mathbf{D}$ is smaller than 1, i.e., $\rho(\mathbf{D}) < 1$. The spectral radius of a square matrix is the maximum of the absolute values of its eigenvalues.
Given this general result, we are able to analyze the convergence condition of AttriInfer.  

\begin{theorem}[Sufficient and Necessary Condition] 
\label{lemma_2}
The sufficient and necessary condition that AttriInfer converges is to bound 
the residual homophily strength $\hat{w}$ as:  
\begin{align}
\label{suff_ness_cond}
\begin{split}
 \hat{w} < \frac{1}{2 \rho(\mathbf{M})}.
\end{split}
\end{align}

\end{theorem}
\begin{proof}
Let $\mathbf{D} = 2\hat{w} \cdot \mathbf{M}$, then $\rho(\mathbf{D})= 2\hat{w} \cdot \rho(\mathbf{M})$.  $\rho(\mathbf{D})< 1$ holds if and only if $\hat{w} < \frac{1}{2\rho (\mathbf{M})}$.
%See Appendix~\ref{app:prooflemma2}.
\end{proof}

Theorem~\ref{lemma_2} provides a strong sufficient and necessary convergence condition.
However, in practice setting $\hat{w}$ using Theorem~\ref{lemma_2} is computationally expensive, as it involves computing the largest eigenvalue with respect to spectral radius. Hence, we instead derive a \emph{sufficient condition} for AttriInfer's convergence, which enables us to set $\hat{w}$  with cheap computation. Specifically, our sufficient condition is based on the fact that any norm is an upper bound of the spectral radius~\cite{derzko1965bounds}, i.e., $\rho(\mathbf{D}) \leq \| \mathbf{D} \|$, where $\| \cdot \|$ indicates some matrix norm. 
In particular, we use the induced $l_1$ matrix norm $\| \cdot \|_1$, where $\| \mathbf{D} \|_1 = \max_{j } \sum_{i} | \mathbf{D}_{ij} | $, the maximum absolute column sum of the matrix. In this way, our sufficient condition for convergence is as follows:

\begin{theorem}[Sufficient Condition] 
\label{lemma_3}
The sufficient condition that AttriInfer converges is
\begin{align}
\label{suff_cond}
\hat{w} < \frac{1}{2\| \mathbf{M} \|_1}=\frac{1}{2\max_{u \in V} d_u}, 
\end{align}
where $d_u=|\Gamma_u|$ is the degree of $u$.
%where $d_u=|\Gamma_u|$ is the number of neighbors of $u$.
\end{theorem}
\begin{proof}
As $\rho(\mathbf{D}) \leq \|\mathbf{D}\|_1$, we achieve the sufficient condition by enforcing $\|\mathbf{D}\|_1 < 1$, where $\mathbf{D} = 2\hat{w} \cdot \mathbf{M}$. Specifically, we have
\begin{align} 
2\hat{w} \cdot \rho(\mathbf{M})  < 1 \Longleftarrow & 2 \hat{w} \|{\bf M}\|_1 < 1 \\
 \Longleftarrow & \hat{w} < \frac{1}{2 \|\mathbf{M}\|_1} = \frac{1}{2 \max_{u\in V} d_u}.
%$2\hat{w} \cdot \rho(\mathbf{A}) \leq 2\hat{w} \|\mathbf{M}\|_1 < 1 \rightrightarrow \hat{w} < \frac{1}{2 \|\mathbf{M}\|_1} = \frac{1}{2 \max_{u\in V} D_u}.$
%See Appendix~\ref{app:prooflemma3}.
\end{align}
\end{proof}

Theorem~\ref{lemma_3} guides us to set $\hat{w}$, i.e., once $\hat{w}$ is smaller than the inverse of 2 times of the maximum node degree, AttriInfer is guaranteed to converge. 
In practice, however, some users (e.g., celebrities) could have orders of magnitude bigger degrees than the others (e.g., ordinary people), and such nodes make $\hat{w}$ very small. 
In our experiments, we find that AttriInfer can still converge when replacing the maximum node degree with the average node degree.

 \subsection{Complexity Analysis}
  We use sparse matrix representation to implement AttriInfer. 
 Computational time of the optimized AttriInfer consists of two parts: time required to compute the prior probabilities using logistic regression, 
 and time required to compute the posterior probabilities via iterative computations.  
The time complexity of the second part is $O(t \cdot |E|)$, where $t$ is the number of iterations.
The time complexity of AttriInfer does not rely on the number of target users whose attributes an attacker wants to infer. 
 We note that the basic version of AttriInfer has the same asymptotic time complexity. 
 However, the constants in the asymptotic representations are different, 
 which results in different scalability. 
 
 VIAL~\cite{GongAttributeInfer16} does not learn the prior probabilities. For each target user, VIAL 
 computes the stationary probability distribution of a random walk in the augmented graph, which starts from the target user. 
 The time complexity of VIAL is $O(t \cdot (|E| + m_1 + m_2) \cdot n_t)$, where $t$ is the number of iterations that a random walk requires to converge, 
 $m_1$ is the total number of public attributes of all users, $m_2$ is the total number of behaviors of all users, and $n_t$ is the number of target users. 
 As we will demonstrate in our experiments, although VIAL does not learn the prior probabilities, it will be orders of magnitude slower than AttriInfer when 
 an attacker aims to infer attributes for a large number of target users. 


==> table.tex <==
\begin{table}[!t]\renewcommand{\arraystretch}{1}
\centering
\caption{Sybil classification on the Twitter dataset. Numbers in the parenthesis are standard deviations.}
\centering
%\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{|c|c|c|} \hline 
{\small False Positive Categories} & {\small # of Accounts} & {\small Percentage} & {\small Notes}\\ \hline
{\small Suspended} & {\small 1} & {\small 0.99\%} & {\small Account suspended by Twitter.}\\ \hline
{\small Deteleted} & {\small 4} & {\small 3.96\%} & {\small Account deleted by user.}\\ \hline
{\small Suspicious} & {\small 1} & {\small 0.99\%} & {\small This user has another social network account. It has been suspended by the service provider. So we consider this user suspicious.}\\ \hline
{\small Commercial} & {\small 36} & {\small 35.64\%} & {\small Accounts in this category are for commercial purposes. They have hundreds of thousands of tweets, most are advertisements or links for commercial use. They tend to follow back whoever follows them. As a result, they have huge numbers of tweets, followings and followers.}\\ \hline
{\small Celebrities} & {\small 18} & {\small 17.82\%} & {\small Accounts in this category are for personal use. Most of the users are celebrities in their community. They generally have hundreds even thousands times of followers than followings.}\\ \hline
{\small Ordinary} & {\small 41} & {\small 40.59\%} & {\small Ordinary Twitter users.}\\ \hline
{\small Total} & {\small 101} & {\small 100.00\%} & {\small FNR}\\ \hline

\end{tabular}
\vspace{-4mm}
\label{falsepos}
\end{table}

